iTelos -- Purpose Driven Knowledge Graph Generation

When building a new application we are more and more confronted with the need of reusing and integrating pre-existing knowledge, e.g., ontologies, schemas, data of any kind, from multiple sources. Nevertheless, it is a fact that this prior knowledge is virtually impossible to reuse as-is. This difficulty is the cause of high costs, with the further drawback that the resulting application will again be hardly reusable. It is a negative loop which consistently reinforces itself. iTelos is a general purpose methodology aiming at minimizing as much as possible the effects of this loop. iTelos is based on the intuition that the data level and the schema level of an application should be developed independently, thus allowing for maximum flexibility in the reuse of the prior knowledge, but under the overall guidance of the needs to be satisfied, formalized as competence queries. This intuition is implemented by codifying all the requirements, including those concerning reuse, as part of an a-priori defined purpose, which is then used to drive a middle-out development process where the application schema and data are continuously aligned.

==> sec_02_soa.tex <==
\section{DI strategies} \label{sec2_soa}

% Data availability increase the need for:

% integrate data in many different domains, defining thus a general purpose demand for integration solutions. 

% such solutions have to be designed to satisfy also very specif purposes

% Specific purpose application
% brings to over fitted structure where organize and maintain integrated data.
% P1 -> no extensible in time
% P2 -> no reusability , negative loop


%The amount of data and relative information, nowadays available, increases the need of integration solutions able to exploit heterogeneous data through single applications/services. We detail in this section, the problem of defining a general purpose DI strategy, able to produce reusable resources. Then the analysis of existing DI strategy is reported, explaining which are the limits of such strategies in solving the problem stated.

%\subsection{The problem}

%The context in which data integration is requested can vary a lot, from business enterprise contexts, collecting data from big data sources like data warehouse and data lakes [CITATIONS], to smaller context such as the management of personal information within your PC. It clearly appears how the purpose for which the integration outcome is produced, changes consequently from one context to one another. Not only the context of data retrieval, but also the exploitation of the integration outcome, increases the number of possible purposes to be considered. In fact, DI integration can be exploited for many different objectives, such as integration of existing data, generation of information structures (databases, KGs) later populated with incoming data, statistical analysis and many other applications in several domains of interest. Such wide range of possible DI purposes, implies difficulties in the definition of standards general purpose methodologies and frameworks.


% increased data availability, and accessibility, leads also to the exploitation of DI for very specific purposes. A perfect example of this scenario are the Personal Management Information system (PIMs)[CITATIONS], used by single persons to integrate their own information. Clearly the application of such systems can have very specific purposes referred to any single aspects of the person's life (i.e. integrate all the information about a single person's vacation, such as photos, videos, notes, GPS traces, and others). The design of such kind of specif purpose services, brings often to model data structures over fitted on data, thus hardly extensible and reusable out of the purpose of their creation. The missing of reusable resources (like data and data schemas) increases, consequently, the effort in data collection and information modelling activities, thus often falling back to the generation of new over fitted resources. It is a negative loop which consistently reinforces itself, producing specif purpose resources, which in turn have to be remodeled from scratch to satisfy new requirements, or extending the original ones. Within the existing data integration strategies, we identified a lack of methodologies and frameworks which can be applied in any possible domain of interest. Moreover, the results obtained by the existing DI solutions, are not reusable enough in different domains (or integration purposes). Due to that the negative reusability loop is not yet broken, thus keeping higher the effort required within the integration process. In support of this claim, we reported, in the next sub section, the analysis of the existing DI strategies, and their limitations with respects the problems expressed above. 



Major improvements in DI have been produced thanks to the studies on Semantic Web. Due to that the ontology-based DI (OBDI) approach \cite{2001-obdi} is now considered for many applications. The key objective of OBDI techniques is to produce a unique representation of the information carried by data provided by different sources. OBDI approach aims to share the data models used by each source with the consequent objective to build a global data model (global ontology) able to provide a unified representation of the data. The existing OBDI strategies can be collected within two different categories, called virtualization and materialization.

\textit{Virtualization strategies} aim to provide a unique view over multiple data sources, without extraction and transformation of their data. That is why they are also known as Ontology Based Data Access (OBDA). Virtualization strategies build a unique view of data, on which the queries are posed, allowing software applications to exploit the integration result. The queries posed to the global view, are then translated into queries on single sources data models, allowing the effective information retrieval. In \cite{2017-obdi-for-mdee} Ekaputra et al. report different DI solutions which differs based on how they produce a global view over multiple data sources. The global view can be build as a single ontology modeled over the different data sources model. Such approach unifies the data sources information but is typically hard to maintain because it is susceptible to changes in each data source. Other OBDA approaches define multiple ontologies, one for each data sources, defining then semantic mapping between them (multiple-ontology OBDI). A different approach, instead, adopts a unique vocabulary to define each single local ontology (hybrid OBDI), simplifying the ontology definition as well as the query building. A composition of the previous solutions has been produced by defining both multiple local ontologies and a single global one, then defining mappings between the local and global layer (\textit{Global-As-View} OBDI). The different OBDA approaches can be in general described by two main features. (i) They integrate the access to data sources more than the data collected within them. (ii) Leaving out the single-ontology approach having more high maintenance cost, OBDA strategies require the definition of multiple ontologies as well as the respective mappings between them. Due to the two features above, OBDA strategies are more suitable for applications which need a unified access to multiple sources than for those exploiting a single information structure, thus having a direct control over the data.


\textit{Materialization strategies} are based on ETL procedures used to extract the data to be integrated from the respective data sources. The subsequent objective is to create a single information structure able to maintain the heterogeneous data collected. Therefore providing a single object for data management and exploitation. Compared with virtualization strategies, materialization ones work directly on data extracted from the sources, building a single global ontology for the data extracted, thus reducing the effort in building multiple ontologies (and relative mappings). Nevertheless, materialization strategies have to deal with the heterogeneity of the data extracted from different sources. Such heterogeneity can be recognized on different levels within the datasets collected, at language level (in case of cross country data integration), at conceptual level (when a real word entity is represent by different properties in different datasets) and at single values level (different data format and standards adopted by different datasets). In \cite{2020-Stratified-DI} Giunchiglia et al. propose an efficient solutions which aims to handle the different levels of heterogeneity through different Knowledge Graphs (KGs). Those KGs are then composed together to build a single object able to maintain and exploit heterogeneous data. More in general the usage of KGs increased a lot within the data integration community, thanks to their exploitability in many different domain of interest, such as sustainable transportation \cite{2021-kg-for-battery}, biomedical data \cite{2021-kg-biomedical} as well as disaster management \cite{2019-KG-embedding}, and many others. DI based on KGs construction (KGC) aims to model a single knowledge representation which must be able to satisfy the integration requirements. The existing KGC-based DI frameworks and tools are defined on single domains of interest, by exploiting a fixed knowledge representation when the global schema is built. In other words, there is always a domain specific ontology, that is used on top to construct the ontology specific for the integration requirements. Some approaches have been proposed considering as base knowledge a more general ontology (allowing suitability for more domains), like \textit{Schema.org}. Adding extensions to the top level ontology, these solutions aim to represent more domain specific aspects required for the integration objective \cite{2020-kg-intro}. Nevertheless this approach produces KGs that are more specific, and less reusable in other domains, the higher is the number of extensions added to the original standard schema (i.e. Schema.org).






